The Green Bank North Celestial Cap Survey. VIII. 21 New Pulsar Timing Solutions

We present timing solutions for 21 pulsars discovered in 350 MHz surveys using the Green Bank Telescope (GBT). All were discovered in the Green Bank North Celestial Cap pulsar survey, with the exception of PSR J0957-0619, which was found in the GBT 350 MHz Drift-scan pulsar survey. The majority of our timing observations were made with the GBT at 820 MHz. With a spin period of 37 ms and a 528-day orbit, PSR J0032+6946 joins a small group of five other mildly recycled wide binary pulsars, for which the duration of recycling through accretion is limited by the length of the companion's giant phase. PSRs J0141+6303 and J1327+3423 are new disrupted recycled pulsars. We incorporate Arecibo observations from the NANOGrav pulsar timing array into our analysis of the latter. We also observed PSR J1327+3423 with the Long Wavelength Array, and our data suggest a frequency-dependent dispersion measure. PSR J0957-0619 was discovered as a rotating radio transient, but is a nulling pulsar at 820 MHz. PSR J1239+3239 is a new millisecond pulsar (MSP) in a 4-day orbit with a low-mass companion. Four of our pulsars already have published timing solutions, which we update in this work: the recycled wide binary PSR J0214+5222, the non-eclipsing black widow PSR J0636+5128, the disrupted recycled pulsar J1434+7257, and the eclipsing binary MSP J1816+4510, which is in an 8.7 hr orbit with a redback-mass companion.

==> binaries_old.tex <==
\begin{splitdeluxetable*}{lrllcccBcccccccc}
  \tabletypesize{\footnotesize}
  \tablewidth{\textwidth}
  \tablecolumns{15}
  \tablecaption{Orbital Parameters for GBNCC Pulsars in Binary Systems}
  \tablehead{
      \colhead{PSR} & \multicolumn{6}{c}{Measured} & \multicolumn{2}{c}{Measured} & \multicolumn{6}{c}{Derived} \\
      \colhead{} &
      \colhead{$\nu_\mathrm{b}$} & 
      \colhead{$a\sin{i}/c$} & 
      \colhead{$T_\mathrm{asc}$} &
      \colhead{$e\sin\omega$} & 
      \colhead{$e\cos\omega$} &
      \colhead{$\dot x$} &
      \colhead{$\dot{\nu}_\mathrm{b}$} & 
      \colhead{$\ddot{\nu}_\mathrm{b}$} & 
      \colhead{$P_\mathrm{b}$} & 
      \colhead{$T_0$} & 
      \colhead{$\omega$} & 
      \colhead{$e$} & 
      \colhead{$f_\mathrm{M}$} & 
      \colhead{$M_\mathrm{c,min}$} \\
      \colhead{} &
      \colhead{(Hz)} &
      \colhead{(s)} &
      \colhead{(MJD)} &
      \colhead{} &
      \colhead{} &
      \colhead{(s\,s$^{-1}$)} &
      \colhead{(Hz\,s$^{-1}$)} &
      \colhead{(Hz\,s$^{-2}$)} &
      \colhead{(days)} &
      \colhead{(MJD)} & 
      \colhead{(\arcdeg)} & 
      \colhead{} & 
      \colhead{(\Msun)} &
      \colhead{(\Msun)}
  }
  \startdata
  J0032+6946 & 2.193632768(6)$\times$10$^{-8}$ & 178.674768(3) & 56399.134959(4) & \phm{$-$}0.00028554(2) & $-$0.00044865(3) &     \ldots & \ldots & \ldots & 527.621316(2)\tphn\dphn & 56615.350(3)\phn & 147.525(2)\phn & 0.00053181(3) & 2.20$\times$10$^{-2}$ & 0.417 \\
  J0214+5222 & 2.260385779(8)$\times$10$^{-8}$ & 174.565762(5) & 56339.115122(4) & $-$0.00271145(5) & $-$0.00458641(6) & \ldots & \ldots & $-$2.1(6)$\times$10$^{-13}$ & 512.039767(2)\tphn\dphn & 56638.6460(8) & 210.5913(6) & 0.00532795(5) & 2.18$\times$10$^{-2}$ & 0.416 \\
  J0636+5128 & 1.739119636(3)$\times$10$^{-4}$ & \dphn0.0089858(1) & 56711.9950666(4) & 1(2)$\times$10$^{-5}$ & $-$1(2)$\times$10$^{-5}$ &     $-$7.1(7)$\times$10$^{-20}$ & $-$2.4(8)$\times$10$^{-27}$ & \ldots & \phn0.0665513392(1) & 56712.02(2)\dphn & 145(106)\dphn\phd & 1(2)$\times$10$^{-5}$ & 1.76$\times$10$^{-7}$ & 0.007 \\
  J1239+3239 & 2.833032117(4)$\times$10$^{-6}$ & \dphn2.371127(2) & 57730.0800015(9) & 5(2)$\times$10$^{-6}$ & \phm{$-$}0(2)$\times$10$^{-6}$ &     \ldots & \ldots & \ldots & 4.085401647(6) & 57731.1(3)\tphn & 89(22)\dphn\phd & 5(2)$\times$10$^{-6}$ & 8.58$\times$10$^{-4}$ & 0.126 \\
  J1816+4510 & 3.2070609894(7)$\times$10$^{-5}$ & \dphn0.5954006(6) & 56945.0911546(2) & 8(2)$\times$10$^{-6}$ & $-$1(2)$\times$10$^{-6}$ &     \ldots & \ldots & \ldots & \dphn0.36089348198(8) & 56945.19(1)\dphn & 97(14)\dphn\phd & 8(2)$\times$10$^{-6}$ & 1.74$\times$10$^{-3}$ & 0.162 \\
  \enddata
  \tablecomments{We report binary parameters for each pulsar in this analysis with evidence of a binary companion. 
  We used the ELL1 binary model for each pulsar, but with two different implementations: for PSRs \psra and \psrc, we implemented Equation~\ref{eq:roemer}, which expresses the Roemer delay up to third order in $e$, in \texttt{PINT}; for the other pulsars, we used the ELL1 binary model as implemented in \tempotwo, which only includes the first-order Roemer-delay terms.
  We report measured orbital frequencies $\nu_\mathrm{b}$, semimajor axes projected along the line of sight, $x=a\sin{i}/c$, times of ascending node $T_\mathrm{asc}$, and first and second Laplace-Lagrange parameters, $e_1 = e\sin\omega$ and $e_2 = e\cos\omega$. 
  We also report first and second derivatives of orbital frequency ($\dot{\nu}_\mathrm{b}$ and $\ddot{\nu}_\mathrm{b}$, respectively), and a time derivative of the projected semimajor axis, $\dot{x}$.
  Using the measured binary parameters, we derive the orbital period $P_\mathrm{b}$, time of periastron $T_0$, longitude of periastron $\omega$, eccentricity $e$, the binary mass function $f_\mathrm{M} = (M_\mathrm{c}\sin i)^3(M_\mathrm{p}+M_\mathrm{c})^{-2}$, and the minimum companion mass $M_\mathrm{c, min} = f_\mathrm{M}(M_\mathrm{p} = 1.4\,\mathrm{M}_\sun, i = 90\arcdeg)$.
  Values in parentheses are the $1$-$\sigma$ uncertainty in the last digit.
  }
\end{splitdeluxetable*}
